New Ideas in Baryogenesis: A Snowmass White Paper

The Standard Model of Particle Physics cannot explain the observed baryon asymmetry of the Universe. This observation is a clear sign of new physics beyond the Standard Model. There have been many recent theoretical developments to address this question. Critically, many new physics models that generate the baryon asymmetry have a wide range of repercussions for many areas of theoretical and experimental particle physics. This white paper provides an overview of such recent theoretical developments with an emphasis on experimental testability.

==> title.tex <==
\begin{titlepage}

\vspace*{-3.5cm}

\noindent

\vspace*{4.0cm}

{\normalfont\bfseries\boldmath\huge
\begin{center}
  \papertitle
\end{center}
}

\vspace*{1.0cm}

\begin{center}
\textbf{Editors:} M. Borsato\ref{hei}, X. Cid Vidal\ref{usc}, Y. Tsai\ref{mar}$^,$\ref{notredame}, C. V\'{a}zquez Sierra\ref{cern}, J. Zurita\ref{ific}

\vspace{1cm}
\textbf{Authors:} 
G.~Alonso-\'{A}lvarez\ref{mcgill}, 
\vspace{1cm}

\end{center}

{\footnotesize
\begin{enumerate}[label = {$^{\arabic*}$}, labelsep = 1pt]
\item Physikalisches Institut, Ruprecht-Karls-Universit\"{a}t Heidelberg, Heidelberg, Germany \label{hei}
\item Instituto Galego de F{\' i}sica de Altas Enerx{\' i}as (IGFAE), Universidade de Santiago de Compostela, Santiago de Compostela, Spain \label{usc}
\item Maryland Center for Fundamental Physics, Department of Physics, University of Maryland, College Park, MD 20742-4111, United States \label{mar}
\item Department of Physics, University of Notre Dame, South Bend, IN 46556, USA \label{notredame}
\item European Organization for Nuclear Research (CERN), Geneva, Switzerland \label{cern}
\item INFN Sezione di Milano, Milano, Italy \label{milano}
\item Instituto de F\'isica Corpuscular (CSIC-UV), Valencia, Spain  \label{ific}
\item McGill University Department of Physics \& McGill Space Institute,
3600 Rue University, Montr\'eal, QC, H3A 2T8, Canada\label{mcgill}
\item Intituut-Lorentz, Leiden University, 2333 CA Leiden, the Netherlands\label{lorentz}
\item Institute for Theoretical Physics, Heidelberg University, 69120 Heidelberg, Germany \label{itphei}
\item Department of Physics, Chalmers University of Technology, Fysikg{\r{a}}rden, 41296 G{\" o}teborg, Sweden \label{chalmers}
\item Physics Department, University of Gothenburg, 41296 G\"oteborg, Sweden \label{goth}
\item University of Lyon, Universit{\' e} Claude Bernard Lyon 1, F-69001 Lyon, France \label{lyon}
\item Institut de Physique des 2 Infinis (IP2I) de Lyon, CNRS/UMR5822, F-69622 Villeurbanne, France \label{lyon2}
\item Department of Physics, Nanjing University, Nanjing 210093, China \label{nanjing} 
 \item Department of Physics, University of Washington, Seattle, WA 98195, USA 
 \label{seattle}
\item Physik-Department, Technische Universit{\" a}t, M{\" u}nchen, James-Franck-Stra{\ss}e, 85748 Garching, Germany \label{tum}



\item Center for Theoretical Physics of the Universe, Institute for Basic Science (IBS), Daejeon 34126, Korea
 \label{IBS}
 \item Institute for Particle Physics Phenomenology,
Durham University, Durham DH1 3LE, United Kingdom \label{ippp}
\item Centre for Cosmology, Particle Physics and Phenomenology,
Universit{\' e} catholique de Louvain, Louvain-la-Neuve B-1348, Belgium  \label{louvain}
\item Department of Physics, Universit{\" a}t Basel, Klingelbergstraße 82, CH-4056 Basel, Switzerland \label{basel}
\item Department of Physics, University of Cincinnati, Cincinnati, Ohio 45221, USA \label{cin}
\item Jo\v{z}ef Stefan Institute, Jamova 39, 1000 Ljubljana, Slovenia \label{jsi}
\item 
Faculty of Mathematics and Physics, University of Ljubljana, Jadranska 19, 1000 Ljubljana, Slovenia 
\label{ljubljana}
\item Institute of Physics, Ecole Polytechnique F{\' e}d{\' e}rale de Lausanne (EPFL), Lausanne, Switzerland \label{epfl}
\item Theoretical Physics Department, Fermilab, P.O. Box 500, Batavia, IL 60510 \label{fnal}
\item Center for High Energy Physics, Peking University, Beijing 100871, China \label{beijing}
\item CAS Center for Excellence in Particle Physics, Beijing 100049, China \label{CAS}
\item Universidade Federal do Rio de Janeiro (UFRJ), Rio de Janeiro, Brazil \label{ufrj}
\item CAFPE and Departamento de F\'isica Te\'orica y del Cosmos, Universidad de Granada,
Campus de Fuentenueva, E–18071 Granada, Spain \label{granada}
\item Laborat\'orio de Instrumenta\c{c}ao e Física Experimental de Partículas, Departamento de Física da Universidade do Minho, Campus de Gualtar, 4710-057 Braga, Portugal \label{minho}
 \item Department of Physics, University of Warwick, Coventry, United Kingdom \label{war}
 \item Istituto Nazionale di Fisica Nucleare (INFN), Padova Division, Padova, Italy \label{pad}
\item Physics Department, Technion – Israel Institute of Technology, Haifa 3200003, Israel \label{technion}
\item Van Swinderen Institute, University of Groningen, Groningen, Netherlands \label{gron}
\item Laboratory for Nuclear Science, Massachusetts Institute of Technology, Cambridge, MA 02139, U.S.A. \label{mit}
\end{enumerate}

%\vspace{\fill}
}

\begin{abstract}
  \noindent
  In this paper, we describe the potential of the LHCb experiment to detect Stealth physics. This refers to dynamics beyond the Standard Model that would elude searches that focus on energetic objects or precision measurements of known processes. Stealth signatures include long-lived particles and light resonances that are produced very rarely or together with overwhelming backgrounds. We will discuss why LHCb is equipped to discover this kind of physics at the Large Hadron Collider and provide examples of well-motivated theoretical models that can be probed with great detail at the experiment.
\end{abstract}

%\vspace*{2.0cm}
\begin{center}
{\tt CP3-21-16, TUM-HEP-1341/21}
\end{center}
\vspace{\fill}

\pagestyle{empty}

\end{titlepage}


\pagestyle{empty}

\newpage
\setcounter{page}{2}
\mbox{~}



